Optimal Charging of an Electric Vehicle Battery Pack: A Real-Time Sensitivity-Based MPC approach

Lithium-ion battery packs are usually composed of hundreds of cells arranged in series and parallel connections. The proper functioning of these complex devices requires suitable Battery Management Systems (BMSs). Advanced BMSs rely on mathematical models to assure safety and high performance. While many approaches have been proposed for the management of single cells, the control of multiple cells has been less investigated and usually relies on simplified models such as equivalent circuit models. This paper addresses the management of a battery pack in which each cell is explicitly modelled as the Single Particle Model with electrolyte and thermal dynamics. A nonlinear Model Predictive Control (MPC) is presented for optimally charging the battery pack while taking voltage and temperature limits on each cell into account. Since the computational cost of nonlinear MPC grows significantly with the complexity of the underlying model, a sensitivity-based MPC (sMPC) is proposed, in which the model adopted is obtained by linearizing the dynamics along a nominal trajectory that is updated over time. The resulting sMPC optimizations are quadratic programs which can be solved in real-time even for large battery packs (e.g. fully electric motorbike with 156 cells) while achieving the same performance of the nonlinear MPC.

==> sec/Conclusions.tex <==
In the present paper, we have proposed a  priority-based model predictive control strategy which relies on the lexicographic approach in order to optimally manage the trade-off between fast charging and ageing reduction in Lithium-ion batteries. Firstly, the equations of a control oriented simplified electrochemical model with thermal and  ageing dynamics are recalled. Then, the advantages of the lexicographic methodology with respect to the conventional MPC, based on a scalar cost function, are highlighted. In particular, we show that this latter is not able to directly represent  the priority order expressed by the decision maker. Furthermore, a modified lexicographic approach suitable for reference tracking MPC problem is considered and   adapted to the charging of a  Lithium-ion cell. In addition, a shrinking-horizon termination method is proposed thus improving the finite-time reachability of the reference target. The results show the effectiveness of the presented algorithm  in terms of charging-time and ageing effects reduction. Finally, with the aim of considering a more realistic scenario, the proposed procedure is tested on the LIONSIMBA simulator and similar results are obtained. In this case, we consider an EKF in order to reconstruct the states vector since only voltage and temperature  are assumed measurable.  

In conclusion, the main contributions of this paper consist in the exploitation of the lexicographic methodology for the first time in the battery context, which results in a significant improvement with respect to standard strategies, and in the addition of the shrinking-horizon termination procedure. 

Future work will be devoted to the use of priority-based methods in the management of a whole battery pack, which is usually constituted by both parallel and series connections of cells. 
